Tropical Jacobians in R2

By tropical Abel-Jacobi theorem, the Jacobian of a tropical curve is isomorphic to the Picard group. A tropical curve in $\mathbb{R}^2$ corresponds to an immersion from a tropical curve to $\mathbb{R}^2$. In this paper, we show that any principal divisor on a tropical curve is the restriction of a principal divisor on the ambient plane $\mathbb{R}^2$.

==> picture/bhA1.tex <==
\begin {picture}(0, 0)
\includegraphics {./picture/bhA1.eps}
\end {picture}
\begin {picture}(350, 150)
\unitlength= 1 mm

\put (28, -5) {$C$}
\put (85, -5) {$\xxBunch(C)$}

\end {picture}


==> picture/bhA3.tex <==
\begin {picture}(0, 0)
\includegraphics {./picture/bhA3.eps}
\end {picture}
\begin {picture}(350, 150)
\unitlength= 1 mm

\put (20, 0) {$C$}
\put (62, 0) {$\xxBunch(C)$}
\put (106, 0) {$\xxNewt(C)$}

\end {picture}


==> picture/bhA4.tex <==
\begin {picture}(0, 0)
\includegraphics {./picture/bhA4.eps}
\end {picture}
\begin {picture}(350, 150)
\unitlength= 1 mm

\put (25, -5) {$C$}
\put (90, 8) {$P$}
\put (100, 40) {$Q$}
\put (86, 2) {$L$}
\put (96, 46) {$M$}

\end {picture}


==> picture/bhA8.tex <==
\begin {picture}(0, 0)
\includegraphics {./picture/bhA8.eps}
\end {picture}
\begin {picture}(350, 150)
\unitlength= 1 mm

\put (26, 37) {$P$}
\put (35, 40) {$P'$}
\put (33, 25) {$R$}
\put (11, 10) {$Q$}
\put (25, 8) {$Q'$}
\put (55, 46) {$S$}
\put (55, 5) {$T$}
\put (4, 42) {$L$}

\put (102, 24) {$\oo$}
\put (91, 29) {$\oo_i$}
%\put (70, 29) {$\Lambda_i$}

\end {picture}

